To Err Is AI! Debugging as an Intervention to Facilitate Appropriate Reliance on AI Systems

Powerful predictive AI systems have demonstrated great potential in augmenting human decision making. Recent empirical work has argued that the vision for optimal human-AI collaboration requires 'appropriate reliance' of humans on AI systems. However, accurately estimating the trustworthiness of AI advice at the instance level is quite challenging, especially in the absence of performance feedback pertaining to the AI system. In practice, the performance disparity of machine learning models on out-of-distribution data makes the dataset-specific performance feedback unreliable in human-AI collaboration. Inspired by existing literature on critical thinking and a critical mindset, we propose the use of debugging an AI system as an intervention to foster appropriate reliance. In this paper, we explore whether a critical evaluation of AI performance within a debugging setting can better calibrate users' assessment of an AI system and lead to more appropriate reliance. Through a quantitative empirical study (N = 234), we found that our proposed debugging intervention does not work as expected in facilitating appropriate reliance. Instead, we observe a decrease in reliance on the AI system after the intervention -- potentially resulting from an early exposure to the AI system's weakness. We explore the dynamics of user confidence and user estimation of AI trustworthiness across groups with different performance levels to help explain how inappropriate reliance patterns occur. Our findings have important implications for designing effective interventions to facilitate appropriate reliance and better human-AI collaboration.

==> sections/sec-rel.tex <==
\section{Related Work}
~\glcomment{Current version is from Abri, I may rewrite all later}
\subsection{Human-AI Decision Making}
~\glcomment{What existing work did? XAI}
Technological advances in the last decade have allowed the use of AI to become a widespread practice for automation in many domains. Practical, ethical, and judicial considerations can make full automation undesirable[1, find efficiency paper, law]. AI, therefore, often has a supporting role by providing predictions to the humans making the final decision. We will refer to this generic process as human-AI decision making. The goal of such joint decision-making is to achieve complementary performance, where human-AI decision making is more accurate than either of its parts separately.

A critical factor in determining this performance is reliance on automation. The widespread usage of AI has incited much research in this area. It has been observed that reliance can be affected by human-, automation-, and context-related factors [3, 4, 5]. In practice, however, the human’s failure to appropriately rely on the system is often the cause of achieving suboptimal performance [6, 7]. This can be described in terms of misuse and disuse, which respectively refer to relying on automation when it performs poorly and rejecting automated predictions when it is correct.

Performant AI solutions often utilize machine learning (ML), which uses functions that are too complex to understand, effectively making them black-box models. Explanations aim to help people understand, appropriately trust, and effectively manage AI [8]. A number of studies support the idea that explanations lead to appropriate reliance by improving human understanding of the AI model [9, 10, 11].


\subsection{Human Mindset Has an Impact on collaboration}
~\glcomment{Provide evidence that our study is meaningful, and potentially}

Human belief systems and decision-making processes can be heavily influenced by the extent to which critical thinking is performed. This complex subject has no universally accepted definition. Different academic disciplines offer their own approaches to defining the subject. To best reflect our concerns, we rely on the work of Robert J. (1986)~\glcomment{add citation} and define critical thinking to be the mental processes, strategies, and representations people use to solve problems, make decisions, and learn new concepts. It is generally agreed upon that critical thinking has both general- and domain-specific aspects [sources]. Some oppose this proposition with some maintaining that critical thinking skills and abilities are not domain-specific [sources], and others that critical thinking skills are purely domain-specific [sources]. Despite this, the importance of domain-specific aspects has been established in much of the existing literature [citations]. By altering these aspects in humans, it is therefore expected to affect their critical thinking.
Prior work has evaluated many domain-specific aspects of Human-AI collaboration, like knowledge, trust, and responsibility. Most researchers agree on the important role of domain-specific knowledge [sources]. As McPeck (1990) notes, to think critically, there needs to be something critical to think about [maybe change quote]. Also, well-established is the role of trust in interaction with technology, with low trust leading to disuse and possible abuse, and high trust potentially causing over-trust which could lead to undesirable outcomes [cite trust paper]. Much research explores the role of responsibility and autonomy in workflows. Results show that increased responsibility leads to performance increases [citations]. Due to its nature, this suggests that critical thinking should improve when this is observed in complex environments. Motivated by this prior work, we propose a way of altering the human mindset~\glcomment{Shall we mention critical mindset consists of all these dimensions?} by improving a human’s understanding of these aspects. By doing this, we hope to increase appropriate reliance between these humans and AI.

\subsection{Trust in AI}
Many studies show that humans interact with technology in a similar fashion as they would with a human collaborator [cite]. Extant research suggests that emotional and attitudinal factors that affect human-to-human interaction may likewise influence human-machine interaction. In these interactions, trust seems to be critically important. In particular, machine reliance appears to be guided by trust [cite tia and their papers], where trusted machines and untrusted machines are likely to be accepted and rejected, respectively. We define trust as suggested by Mayer et al. (1995) to be “the willingness of a party to be vulnerable to the actions of another party based on the expectation that the other will perform a particular action important to the trustor, irrespective of the ability to monitor or control that other party”. As the focus of this research is human-AI collaboration, humans will assume the role of the trustor, and AI systems the role of trustee. Many studies have shown that AI systems used as decision support systems are initially highly trusted, which decreases when erroneous behavior is observed [cite]. Restoring this trust tends to be a lengthy process. This can be mitigated by communicating the AI’s rationale and abilities to the user, which lowers the impractically high initial trust and increases the recovery rate of trust after erroneous behavior is encountered [cite]. We, therefore, propose a training phase aimed at better calibrating user expectations of the AI through a debugging exercise.

